Joint Channel Selection using FedDRL in V2X

Vehicle-to-everything (V2X) communication technology is revolutionizing transportation by enabling interactions between vehicles, devices, and infrastructures. This connectivity enhances road safety, transportation efficiency, and driver assistance systems. V2X benefits from Machine Learning, enabling real-time data analysis, better decision-making, and improved traffic predictions, making transportation safer and more efficient. In this paper, we study the problem of joint channel selection, where vehicles with different technologies choose one or more Access Points (APs) to transmit messages in a network. In this problem, vehicles must learn a strategy for channel selection, based on observations that incorporate vehicles' information (position and speed), network and communication data (Signal-to-Interference-plus-Noise Ratio from past communications), and environmental data (road type). We propose an approach based on Federated Deep Reinforcement Learning (FedDRL), which enables each vehicle to benefit from other vehicles' experiences. Specifically, we apply the federated Proximal Policy Optimization (FedPPO) algorithm to this task. We show that this method improves communication reliability while minimizing transmission costs and channel switches. The efficiency of the proposed solution is assessed via realistic simulations, highlighting the potential of FedDRL to advance V2X technology.

==> images/rl.tex <==
\tikzstyle{block} = [rectangle, draw, 
    text width=8em, text centered, rounded corners, minimum height=4em]
    
\tikzstyle{line} = [draw, -latex]

\begin{tikzpicture}[node distance = 6em, auto, thick]
    \node [block] (Agent) {Agent};
    \node [block, below of=Agent] (Environment) {Environment};
    
     \path [line] (Agent.0) --++ (4em,0em) |- node [near start]{Action $a_t$} (Environment.0);
     \path [line] (Environment.190) --++ (-6em,0em) |- node [near start] {New state  $s_{t+1}$} (Agent.170);
     \path [line] (Environment.170) --++ (-4.25em,0em) |- node [near start, right] {Reward $r_{t+1}$} (Agent.190);
\end{tikzpicture}

==> tables/actions.tex <==
\begin{tabular}{cc}
    \toprule
    \textbf{Label} & \textbf{Action} \\
    \midrule
     0 & No transmission  \\
     1 & DSRC  \\
     2 & VLC Headlight  \\
     3 & DSRC \& Headlight \\
     4 & VLC Taillight  \\
     5 & DSRC \& Taillight \\
     6 & Taillight \& Headlight \\
     7 & DSRC \& Headlight \& Taillight  \\
    \bottomrule
\end{tabular}

==> tables/baselines.tex <==
\begin{tabular}{ccccc} 
\toprule
\multicolumn{1}{l}{} & Scenario 1 & Scenario 2 & Scenario 3  \\
PPO test reward  & 1250          & -          & -           \\
PPO reliability  & 0.625          & -          & -           \\
\midrule
FedPPO reward & \textbf{1462}          & -          & -           \\
FedPPO reliability & \textbf{0.698}         & -          & -           \\

\bottomrule
\end{tabular}

==> tables/experiments-done.tex <==
\begin{tabular}{lcc|cc|ccc} 
\toprule
            & \multicolumn{2}{c}{Scenario 1}                  & \multicolumn{2}{c}{Scenario 2}                    & \multicolumn{3}{c}{Scenario 3}                                                \\
            \midrule
Client      & 1                        & 2                      & 1                        & 2                        & 1                        & 2                        & 3                         \\
Agent       & \follower & \leader & \follower & \follower & \follower & \follower & \follower  \\
Route       & Countryside               & Countryside             & Countryside               & Mountain                & Countryside               & Mountain                & City                 \\
Bg. Traffic & \no       & \no     & \yes      & \yes      & \yes      & \yes      & \yes       \\
\bottomrule
\end{tabular}



==> tables/hyperparameters.tex <==
\begin{tabular}{c|c}
\toprule
        \textbf{Parameter}           &  \textbf{Value}\\
\midrule
        Simulation time     &  $15$ s\\
        Observation space dimension & $15$\\
        Action space dimension & $8$\\
        %Architecture & $64 \times 64$ \\
        Communication cost (DSRC / VLC) & $0.1 / 0.01$\\
        Switching penalty $P$ & $0.01$ \\
        Number of clients & $\{30, 60\}$ \\
        
\bottomrule
\end{tabular}

==> tables/hyperparameters1.tex <==
\begin{tabular}{cc|cc}
%\begin{tabular}
    \toprule
    \textbf{Network parameters} & \textbf{Value} & \textbf{FedPPO parameters} & \textbf{Value} \\
    \midrule
        Hidden layers & $\{1, 2, \mathbf{3}\}$ & Discount factor $\gamma$ & $0.99$\\
        Layer dimension & $64$ & GAE parameter $\lambda$ & $0.95$ \\
        Step size Actors & $ \{3e^{-2}, {1e^{-3}}, \mathbf{5e^{-4}}, 3e^{-5}\} $ & Number of epochs  & $20$\\
        Step size Critics & $ \{ 1e^{-2}, \mathbf{5e^{-3}}, 31e^{-4}, 3e^{-5}\} $ & Number of local steps & $15$\\
        Optimizer Actors & \textbf{Adam}, SGD & Number of rollouts $M$ & $\{5, 8, \textbf{10}\}$\\
        Optimizer Critics & \textbf{Adam}, SGD & Mini-batch size $B$ & $\{256, \mathbf{400}\}$\\  
        Activation function & \textbf{Tanh}, ReLU &  Clip parameter $\epsilon$ & $\{0.1, \mathbf{0.2}, 0.3 \}$\\
     \bottomrule
\end{tabular}

==> tables/scenario1.tex <==
\begin{tabular}{ccccc}
\toprule
     Environment & Agent & Route & Bg. Traffic & Aggregation\\
\midrule
    \multirow{2}{*}{1}  & \multirow{2}{*}{\follower} & \multirow{2}{*}{\textit{Serpentine}} & \multirow{2}{*}{\no} & \\
    & & & &FedAvg \\
    2  & \leader   & \textit{Serpentine} & \no & \\
\bottomrule
\end{tabular}

==> tables/scenario2.tex <==
\begin{tabular}{ccccc}
\toprule
     Environment & Agent & Route & Bg. Traffic & Aggregation\\
\midrule
    \multirow{2}{*}{1}  & \multirow{2}{*}{\follower} & \multirow{2}{*}{\textit{Serpentine}} & \multirow{2}{*}{\yes} & \\
    & & & &FedAvg \\
    2  & \follower   & \textit{Lysevegen} & \yes & \\
\bottomrule
\end{tabular}

==> tables/scenario3.tex <==
\begin{tabular}{ccccc}
\toprule
     Environment & Agent & Route & Bg. Traffic & Aggregation\\
\midrule
    \multirow{2}{*}{1}  & \multirow{2}{*}{\follower} & \multirow{2}{*}{\textit{Serpentine}} & \multirow{2}{*}{\yes} & \\
    & & & & \\
    \multirow{2}{*}{2}  & \multirow{2}{*}{\follower} & \multirow{2}{*}{\textit{Lysevegen}} & \multirow{2}{*}{\yes} & FedAvg \\
    & & & & \\
    \multirow{2}{*}{3}  & \multirow{2}{*}{\follower} & \multirow{2}{*}{\textit{Manhattan}} & \multirow{2}{*}{\yes} & \\
    & & & & \\
\bottomrule
\end{tabular}


==> tables/telecom-parameters.tex <==
\begin{tabular}{c|c}
\toprule
    \textbf{Parameter}   &  \textbf{Value}\\
\midrule
    Beaconing Frequency       &  10 Hz\\
    Packet Byte length        &  1024 byte\\
    Transmission power (DSRC) & 20 mW \\
    Bitrate (DSRC / VLC)    & 6 Mbps / 1 Mbps  \\
    \bottomrule
    
\end{tabular}

==> tables1/tables/experiments-done.tex <==
\begin{tabular}{lcc|cc|ccc} 
\toprule
            & \multicolumn{2}{c}{Scenario 1}                  & \multicolumn{2}{c}{Scenario 2}                    & \multicolumn{3}{c}{Scenario 3}                                                \\
            \midrule
Client      & 1                        & 2                      & 1                        & 2                        & 1                        & 2                        & 3                         \\
Agent       & \follower & \leader & \follower & \follower & \follower & \follower & \follower  \\
Route       & Countryside               & Countryside             & Countryside               & Mountain                & Countryside               & Mountain                & City                 \\
Bg. Traffic & \no       & \no     & \yes      & \yes      & \yes      & \yes      & \yes       \\
\bottomrule
\end{tabular}



==> tables1/tables/hyperparameters.tex <==
\begin{tabular}{c|c}
\toprule
        \textbf{Parameter}           &  \textbf{Value}\\
\midrule
        Simulation time     &  $15$ s\\
        Observation space dimension & $15$\\
        Action space dimension & $8$\\
        %Architecture & $64 \times 64$ \\
        Communication cost (DSRC / VLC) & $0.1 / 0.01$\\
        Switching penalty $P$ & $0.01$ \\
        Number of clients & $\{30, 60\}$ \\
        
\bottomrule
\end{tabular}

==> tables1/tables/hyperparameters1.tex <==
\begin{tabular*}{\textwidth}{@{\extracolsep{\fill}} cc|cc }
%\begin{tabular}{cc|cc}
    \toprule
    \textbf{Network parameters} & \textbf{Value} & \textbf{FedPPO parameters} & \textbf{Value} \\
    \midrule
        Hidden layers & $\{1, 2, \mathbf{3}\}$ & Discount factor $\gamma$ & $0.99$\\
        Layer dimension & $64$ & GAE parameter $\lambda$ & $0.95$ \\
        Step size Actors & $ \{3e^{-2}, {1e^{-3}}, \mathbf{5e^{-4}}, 3e^{-5}\} $ & Number of epochs  & $20$\\
        Step size Critics & $ \{ 1e^{-2}, \mathbf{5e^{-3}}, 31e^{-4}, 3e^{-5}\} $ & Number of local steps & $15$\\
        Optimizer Actors & \textbf{Adam}, SGD & Number of rollouts $M$ & $\{5, 8, \textbf{10}\}$\\
        Optimizer Critics & \textbf{Adam}, SGD & Mini-batch size $B$ & $\{256, \mathbf{400}\}$\\  
        Activation function & \textbf{Tanh}, ReLU &  Clip parameter $\epsilon$ & $\{0.1, \mathbf{0.2}, 0.3 \}$\\
     \bottomrule
\end{tabular*}

==> tables1/tables/routes.tex <==
\begin{tabular*}{\textwidth}{@{\extracolsep{\fill}} cccc }
\toprule
        \textbf{Parameter} & 
        \textbf{Countryside}  &  \textbf{Highway} & \textbf{Urban}\\
\midrule
        Speed of vehicles     & $\sim 20 $ (m/s) &  $\sim 30 $ (m/s) & $\sim 15 $ (m/s)\\
        Background traffic density  & $0-2000$ & $0-2000$ & $0-2000$\\
\bottomrule
\end{tabular*}

==> tables1/tables/scenario1.tex <==
\begin{tabular}{ccccc}
\toprule
     Environment & Agent & Route & Bg. Traffic & Aggregation\\
\midrule
    \multirow{2}{*}{1}  & \multirow{2}{*}{\follower} & \multirow{2}{*}{\textit{Serpentine}} & \multirow{2}{*}{\no} & \\
    & & & &FedAvg \\
    2  & \leader   & \textit{Serpentine} & \no & \\
\bottomrule
\end{tabular}

==> tables1/tables/scenario2.tex <==
\begin{tabular}{ccccc}
\toprule
     Environment & Agent & Route & Bg. Traffic & Aggregation\\
\midrule
    \multirow{2}{*}{1}  & \multirow{2}{*}{\follower} & \multirow{2}{*}{\textit{Serpentine}} & \multirow{2}{*}{\yes} & \\
    & & & &FedAvg \\
    2  & \follower   & \textit{Lysevegen} & \yes & \\
\bottomrule
\end{tabular}

==> tables1/tables/scenario3.tex <==
\begin{tabular}{ccccc}
\toprule
     Environment & Agent & Route & Bg. Traffic & Aggregation\\
\midrule
    \multirow{2}{*}{1}  & \multirow{2}{*}{\follower} & \multirow{2}{*}{\textit{Serpentine}} & \multirow{2}{*}{\yes} & \\
    & & & & \\
    \multirow{2}{*}{2}  & \multirow{2}{*}{\follower} & \multirow{2}{*}{\textit{Lysevegen}} & \multirow{2}{*}{\yes} & FedAvg \\
    & & & & \\
    \multirow{2}{*}{3}  & \multirow{2}{*}{\follower} & \multirow{2}{*}{\textit{Manhattan}} & \multirow{2}{*}{\yes} & \\
    & & & & \\
\bottomrule
\end{tabular}


==> tables1/tables/telecom-parameters.tex <==
\begin{tabular}{c|c}
\toprule
    \textbf{Parameter}   &  \textbf{Value}\\
\midrule
    Beaconing Frequency       &  10 Hz\\
    Packet Byte length        &  1024 byte\\
    Transmission power (DSRC) & 20 mW \\
    Bitrate (DSRC / VLC)    & 6 Mbps / 1 Mbps  \\
    \bottomrule
    
\end{tabular}
